Trustworthy Social Bias Measurement

How do we design measures of social bias that we trust? While prior work has introduced several measures, no measure has gained widespread trust: instead, mounting evidence argues we should distrust these measures. In this work, we design bias measures that warrant trust based on the cross-disciplinary theory of measurement modeling. To combat the frequently fuzzy treatment of social bias in NLP, we explicitly define social bias, grounded in principles drawn from social science research. We operationalize our definition by proposing a general bias measurement framework DivDist, which we use to instantiate 5 concrete bias measures. To validate our measures, we propose a rigorous testing protocol with 8 testing criteria (e.g. predictive validity: do measures predict biases in US employment?). Through our testing, we demonstrate considerable evidence to trust our measures, showing they overcome conceptual, technical, and empirical deficiencies present in prior measures.

==> tables/gender_correlations.GloVe.table.tex <==
\begin{table}[t]
\tiny
\centering
% \renewcommand\arraystretch{1.3}
% \renewcommand\tabcolsep{0pt}
\begin{tabular}{ccccc}
    \toprule
Measure & $\rho$ & $p$ & $R^2$ & $p$ \\
\midrule
garg-cosine & 0.327 & 0.001 & 0.106 & 0.001 \\
garg-euclidean & 0.292 & 0.004 & 0.075 & 0.007 \\
caliskan & 0.295 & 0.003 & 0.088 & 0.003 \\
manzini & -0.082 & 0.423 & 0.009 & 0.361 \\
bolukbasi-conventional & 0.08 & 0.438 & 0.007 & 0.415 \\
ethayarajh-conventional & 0.067 & 0.513 & 0.007 & 0.424 \\
\midrule 
('L1', 'sum', 'cosine') & 0.332 & 0.001 & 0.005 & 0.474 \\
('L1', 'sum', 'inner-product') & 0.244 & 0.016 & 0.001 & 0.769 \\
('L1', 'softmax', 'cosine') & 0.327 & 0.001 & 0.106 & 0.001 \\
('L1', 'softmax', 'inner-product') & 0.247 & 0.015 & 0.051 & 0.026 \\
('L2', 'sum', 'cosine') & 0.332 & 0.001 & 0.005 & 0.474 \\
('L2', 'sum', 'inner-product') & 0.244 & 0.016 & 0.001 & 0.769 \\
('L2', 'softmax', 'cosine') & 0.327 & 0.001 & 0.106 & 0.001 \\
('L2', 'softmax', 'inner-product') & 0.247 & 0.015 & 0.051 & 0.026 \\
('Linf', 'sum', 'cosine') & 0.332 & 0.001 & 0.005 & 0.474 \\
('Linf', 'sum', 'inner-product') & 0.244 & 0.016 & 0.001 & 0.769 \\
('Linf', 'softmax', 'cosine') & 0.327 & 0.001 & 0.106 & 0.001 \\
('Linf', 'softmax', 'inner-product') & 0.247 & 0.015 & 0.051 & 0.026 \\
('KL', 'sum', 'cosine') & 0.334 & 0.001 & nan & nan \\
('KL', 'sum', 'inner-product') & 0.246 & 0.015 & nan & nan \\
('KL', 'softmax', 'cosine') & 0.327 & 0.001 & 0.077 & 0.006 \\
('KL', 'softmax', 'inner-product') & 0.247 & 0.015 & 0.068 & 0.01 \\
('JS', 'sum', 'cosine') & 0.334 & 0.001 & nan & nan \\
('JS', 'sum', 'inner-product') & 0.246 & 0.015 & nan & nan \\
('JS', 'softmax', 'cosine') & 0.327 & 0.001 & 0.106 & 0.001 \\
('JS', 'softmax', 'inner-product') & 0.247 & 0.015 & 0.058 & 0.017 \\
\bottomrule 
\end{tabular}
  \caption{Correlation between measured binary gender bias in pretrained GloVe representations and bias in census statistics from 2010. Targets are all professions with statistics reported in the 2010 census data of \citet{levanon2009}. $\rho$ indicates the Spearman correlation (measure of monotonic correlation) and $R^2$ corresponds to regression via ordinary least-squares (measure of linear correlation); corresponding $p$-values in the column directly to the right.}
  \label{tab:glovegender}
\end{table}

==> tables/gender_correlations.table.tex <==
\begin{table}[t]
\tiny
\centering
% \renewcommand\arraystretch{1.3}
% \renewcommand\tabcolsep{0pt}
\begin{tabular}{ccccc}
\toprule
Measure & $\rho$ & $p$ & $R^2$ & $p$ \\
\midrule
garg-cosine & 0.758 & 0.011 & 0.555 & 0.013 \\
garg-euclidean & 0.127 & 0.726 & 0.219 & 0.172 \\
caliskan & 0.709 & 0.022 & 0.463 & 0.03 \\
manzini & -0.648 & 0.043 & 0.597 & 0.009 \\
bolukbasi-conventional & 0.261 & 0.467 & 0.001 & 0.93 \\
ethayarajh-conventional & 0.261 & 0.467 & 0.001 & 0.93 \\
\midrule 
('L1', 'sum', 'cosine') & 0.83 & 0.003 & 0.249 & 0.142 \\
('L1', 'sum', 'inner-product') & 0.685 & 0.029 & 0.25 & 0.141 \\
('L1', 'softmax', 'cosine') & 0.758 & 0.011 & 0.553 & 0.014 \\
('L1', 'softmax', 'inner-product') & 0.709 & 0.022 & 0.462 & 0.031 \\
('L2', 'sum', 'cosine') & 0.83 & 0.003 & 0.249 & 0.142 \\
('L2', 'sum', 'inner-product') & 0.685 & 0.029 & 0.25 & 0.141 \\
('L2', 'softmax', 'cosine') & 0.758 & 0.011 & 0.553 & 0.014 \\
('L2', 'softmax', 'inner-product') & 0.709 & 0.022 & 0.462 & 0.031 \\
('Linf', 'sum', 'cosine') & 0.83 & 0.003 & 0.249 & 0.142 \\
('Linf', 'sum', 'inner-product') & 0.685 & 0.029 & 0.25 & 0.141 \\
('Linf', 'softmax', 'cosine') & 0.758 & 0.011 & 0.553 & 0.014 \\
('Linf', 'softmax', 'inner-product') & 0.709 & 0.022 & 0.462 & 0.031 \\
('KL', 'sum', 'cosine') & nan & nan & nan & nan \\
('KL', 'sum', 'inner-product') & nan & nan & nan & nan \\
('KL', 'softmax', 'cosine') & 0.879 & 0.001 & 0.664 & 0.004 \\
('KL', 'softmax', 'inner-product') & 0.782 & 0.008 & 0.632 & 0.006 \\
('JS', 'sum', 'cosine') & nan & nan & nan & nan \\
('JS', 'sum', 'inner-product') & nan & nan & nan & nan \\
('JS', 'softmax', 'cosine') & 0.758 & 0.011 & 0.554 & 0.014 \\
('JS', 'softmax', 'inner-product') & 0.709 & 0.022 & 0.463 & 0.03 \\
\bottomrule 
\end{tabular}
  \caption{Correlation between measured binary gender bias in Word2Vec embeddings learned on historic COHA data and bias in diachronic census statistics across the ten decades from 1900 to 2000. Targets are all professions with statistics reported in every census from 1900 to 2000 \citep{levanon2009}. $\rho$ indicates the Spearman correlation (measure of monotonic correlation) and $R^2$ corresponds to regression via ordinary least-squares (measure of linear correlation); corresponding $p$-values in the column directly to the right.}
  \label{tab:diachronicgender}
\end{table}

==> tables/gender_correlations.w2v.table.tex <==
\begin{table}[t]
\tiny
\centering
% \renewcommand\arraystretch{1.3}
% \renewcommand\tabcolsep{0pt}
\begin{tabular}{ccccc}
    \toprule
Measure & $\rho$ & $p$ & $R^2$ & $p$ \\
\midrule
garg-cosine & 0.633 & 0.0 & 0.401 & 0.0 \\
garg-euclidean & 0.553 & 0.0 & 0.306 & 0.0 \\
caliskan & 0.505 & 0.0 & 0.274 & 0.0 \\
manzini & 0.193 & 0.059 & 0.036 & 0.061 \\
bolukbasi-conventional & 0.047 & 0.647 & 0.004 & 0.55 \\
ethayarajh-conventional & 0.065 & 0.524 & 0.007 & 0.419 \\
\midrule 
('L1', 'sum', 'cosine') & 0.42 & 0.0 & 0.033 & 0.074 \\
('L1', 'sum', 'inner-product') & 0.221 & 0.029 & 0.007 & 0.415 \\
('L1', 'softmax', 'cosine') & 0.633 & 0.0 & 0.401 & 0.0 \\
('L1', 'softmax', 'inner-product') & 0.405 & 0.0 & 0.197 & 0.0 \\
('L2', 'sum', 'cosine') & 0.42 & 0.0 & 0.033 & 0.074 \\
('L2', 'sum', 'inner-product') & 0.221 & 0.029 & 0.007 & 0.415 \\
('L2', 'softmax', 'cosine') & 0.633 & 0.0 & 0.401 & 0.0 \\
('L2', 'softmax', 'inner-product') & 0.405 & 0.0 & 0.197 & 0.0 \\
('Linf', 'sum', 'cosine') & 0.42 & 0.0 & 0.033 & 0.074 \\
('Linf', 'sum', 'inner-product') & 0.221 & 0.029 & 0.007 & 0.415 \\
('Linf', 'softmax', 'cosine') & 0.633 & 0.0 & 0.401 & 0.0 \\
('Linf', 'softmax', 'inner-product') & 0.405 & 0.0 & 0.197 & 0.0 \\
('KL', 'sum', 'cosine') & 0.42 & 0.0 & nan & nan \\
('KL', 'sum', 'inner-product') & 0.221 & 0.029 & nan & nan \\
('KL', 'softmax', 'cosine') & 0.633 & 0.0 & 0.335 & 0.0 \\
('KL', 'softmax', 'inner-product') & 0.405 & 0.0 & 0.148 & 0.0 \\
('JS', 'sum', 'cosine') & 0.42 & 0.0 & nan & nan \\
('JS', 'sum', 'inner-product') & 0.221 & 0.029 & nan & nan \\
('JS', 'softmax', 'cosine') & 0.633 & 0.0 & 0.401 & 0.0 \\
('JS', 'softmax', 'inner-product') & 0.405 & 0.0 & 0.195 & 0.0 \\
\bottomrule 
\end{tabular}
  \caption{Correlation between measured binary gender bias in pretrained Word2Vec representations and bias in census statistics from 2010. Targets are all professions with statistics reported in the 2010 census data of \citet{levanon2009}. $\rho$ indicates the Spearman correlation (measure of monotonic correlation) and $R^2$ corresponds to regression via ordinary least-squares (measure of linear correlation); corresponding $p$-values in the column directly to the right.}
  \label{tab:w2vgender}
\end{table}

==> tables/race_correlations.GloVe.table.tex <==
\begin{table}[t]
\tiny
\centering
% \renewcommand\arraystretch{1.3}
% \renewcommand\tabcolsep{0pt}
\begin{tabular}{ccccc}
    \toprule
Measure & $\rho$ & $p$ & $R^2$ & $p$ \\
\midrule
manzini & 0.037 & 0.719 & 0.001 & 0.816 \\
\midrule 
('L1', 'sum', 'cosine') & -0.185 & 0.069 & 0.016 & 0.223 \\
('L1', 'sum', 'inner-product') & -0.188 & 0.065 & 0.0 & 0.87 \\
('L1', 'softmax', 'cosine') & -0.111 & 0.278 & 0.086 & 0.003 \\
('L1', 'softmax', 'inner-product') & -0.194 & 0.057 & 0.069 & 0.01 \\
('L2', 'sum', 'cosine') & -0.19 & 0.063 & 0.016 & 0.215 \\
('L2', 'sum', 'inner-product') & -0.196 & 0.054 & 0.0 & 0.87 \\
('L2', 'softmax', 'cosine') & -0.117 & 0.254 & 0.088 & 0.003 \\
('L2', 'softmax', 'inner-product') & -0.19 & 0.062 & 0.069 & 0.009 \\
('Linf', 'sum', 'cosine') & -0.185 & 0.069 & 0.016 & 0.223 \\
('Linf', 'sum', 'inner-product') & -0.188 & 0.065 & 0.0 & 0.87 \\
('Linf', 'softmax', 'cosine') & -0.111 & 0.278 & 0.086 & 0.003 \\
('Linf', 'softmax', 'inner-product') & -0.194 & 0.057 & 0.069 & 0.01 \\
('KL', 'sum', 'cosine') & -0.189 & 0.063 & nan & nan \\
('KL', 'sum', 'inner-product') & -0.197 & 0.054 & nan & nan \\
('KL', 'softmax', 'cosine') & -0.115 & 0.261 & 0.076 & 0.006 \\
('KL', 'softmax', 'inner-product') & -0.163 & 0.111 & 0.051 & 0.026 \\
('JS', 'sum', 'cosine') & -0.198 & 0.052 & nan & nan \\
('JS', 'sum', 'inner-product') & -0.199 & 0.051 & nan & nan \\
('JS', 'softmax', 'cosine') & -0.116 & 0.257 & 0.088 & 0.003 \\
('JS', 'softmax', 'inner-product') & -0.15 & 0.142 & 0.057 & 0.018 \\
\bottomrule 
\end{tabular}
  \caption{Correlation between measured three-class (White, Hispanic, Asian) race bias in pretrained GloVe representations and bias in census statistics from 2010. Targets are all professions with statistics reported in the 2010 census data of \citet{levanon2009}. $\rho$ indicates the Spearman correlation (measure of monotonic correlation) and $R^2$ corresponds to regression via ordinary least-squares (measure of linear correlation); corresponding $p$-values in the column directly to the right.}
  \label{tab:gloverace}
\end{table}

==> tables/race_correlations.table.tex <==
\begin{table}[t]
\tiny
\centering
% \renewcommand\arraystretch{1.3}
% \renewcommand\tabcolsep{0pt}
\begin{tabular}{ccccc}
    \toprule
Measure & $\rho$ & $p$ & $R^2$ & $p$ \\
\midrule
manzini & -0.903 & 0.0 & 0.787 & 0.001 \\
\midrule 
('L1', 'sum', 'cosine') & 0.842 & 0.002 & 0.217 & 0.175 \\
('L1', 'sum', 'inner-product') & 0.927 & 0.0 & 0.543 & 0.015 \\
('L1', 'softmax', 'cosine') & 0.527 & 0.117 & 0.082 & 0.422 \\
('L1', 'softmax', 'inner-product') & 0.588 & 0.074 & 0.16 & 0.252 \\
('L2', 'sum', 'cosine') & 0.855 & 0.002 & 0.219 & 0.172 \\
('L2', 'sum', 'inner-product') & 0.891 & 0.001 & 0.563 & 0.012 \\
('L2', 'softmax', 'cosine') & 0.527 & 0.117 & 0.08 & 0.428 \\
('L2', 'softmax', 'inner-product') & 0.539 & 0.108 & 0.158 & 0.256 \\
('Linf', 'sum', 'cosine') & 0.842 & 0.002 & 0.217 & 0.175 \\
('Linf', 'sum', 'inner-product') & 0.927 & 0.0 & 0.543 & 0.015 \\
('Linf', 'softmax', 'cosine') & 0.527 & 0.117 & 0.082 & 0.422 \\
('Linf', 'softmax', 'inner-product') & 0.588 & 0.074 & 0.16 & 0.252 \\
('KL', 'sum', 'cosine') & 0.731 & 0.016 & nan & nan \\
('KL', 'sum', 'inner-product') & 0.731 & 0.016 & nan & nan \\
('KL', 'softmax', 'cosine') & 0.612 & 0.06 & 0.09 & 0.401 \\
('KL', 'softmax', 'inner-product') & 0.636 & 0.048 & 0.171 & 0.235 \\
('JS', 'sum', 'cosine') & 0.705 & 0.023 & nan & nan \\
('JS', 'sum', 'inner-product') & 0.731 & 0.016 & nan & nan \\
('JS', 'softmax', 'cosine') & 0.442 & 0.2 & 0.076 & 0.439 \\
('JS', 'softmax', 'inner-product') & 0.539 & 0.108 & 0.144 & 0.279 \\
\bottomrule 
\end{tabular}
  \caption{Correlation between measured three-class (White, Hispanic, Asian) race bias in Word2Vec embeddings learned on historic COHA data and bias in diachronic census statistics across the ten decades from 1900 to 2000. Targets are all professions with statistics reported in every census from 1900 to 2000 \citep{levanon2009}. $\rho$ indicates the Spearman correlation (measure of monotonic correlation) and $R^2$ corresponds to regression via ordinary least-squares (measure of linear correlation); corresponding $p$-values in the column directly to the right.}
  \label{tab:diachronicrace}
\end{table}


==> tables/race_correlations.w2v.table.tex <==
\begin{table}[t]
\tiny
\centering
% \renewcommand\arraystretch{1.3}
% \renewcommand\tabcolsep{0pt}
\begin{tabular}{ccccc}
    \toprule
Measure & $\rho$ & $p$ & $R^2$ & $p$ \\
\midrule
manzini & -0.396 & 0.0 & 0.118 & 0.001 \\
\midrule 
('L1', 'sum', 'cosine') & 0.369 & 0.0 & 0.012 & 0.29 \\
('L1', 'sum', 'inner-product') & 0.423 & 0.0 & 0.02 & 0.165 \\
('L1', 'softmax', 'cosine') & -0.03 & 0.773 & 0.001 & 0.751 \\
('L1', 'softmax', 'inner-product') & 0.082 & 0.425 & 0.007 & 0.432 \\
('L2', 'sum', 'cosine') & 0.369 & 0.0 & 0.011 & 0.304 \\
('L2', 'sum', 'inner-product') & 0.417 & 0.0 & 0.02 & 0.169 \\
('L2', 'softmax', 'cosine') & -0.03 & 0.771 & 0.001 & 0.769 \\
('L2', 'softmax', 'inner-product') & 0.085 & 0.41 & 0.007 & 0.43 \\
('Linf', 'sum', 'cosine') & 0.369 & 0.0 & 0.012 & 0.29 \\
('Linf', 'sum', 'inner-product') & 0.423 & 0.0 & 0.02 & 0.165 \\
('Linf', 'softmax', 'cosine') & -0.03 & 0.773 & 0.001 & 0.751 \\
('Linf', 'softmax', 'inner-product') & 0.082 & 0.425 & 0.007 & 0.432 \\
('KL', 'sum', 'cosine') & 0.386 & 0.0 & nan & nan \\
('KL', 'sum', 'inner-product') & 0.431 & 0.0 & nan & nan \\
('KL', 'softmax', 'cosine') & -0.03 & 0.768 & 0.0 & 0.868 \\
('KL', 'softmax', 'inner-product') & 0.08 & 0.437 & 0.004 & 0.563 \\
('JS', 'sum', 'cosine') & 0.381 & 0.0 & nan & nan \\
('JS', 'sum', 'inner-product') & 0.429 & 0.0 & nan & nan \\
('JS', 'softmax', 'cosine') & -0.03 & 0.769 & 0.001 & 0.76 \\
('JS', 'softmax', 'inner-product') & 0.076 & 0.457 & 0.005 & 0.477 \\
\bottomrule 
\end{tabular}
  \caption{Correlation between measured three-class (White, Hispanic, Asian) race bias in pretrained Word2Vec representations and bias in census statistics from 2010. Targets are all professions with statistics reported in the 2010 census data of \citet{levanon2009}. $\rho$ indicates the Spearman correlation (measure of monotonic correlation) and $R^2$ corresponds to regression via ordinary least-squares (measure of linear correlation); corresponding $p$-values in the column directly to the right.}
  \label{tab:w2vrace}
\end{table}
